Computer-Vision Based Real Time Waypoint Generation for Autonomous Vineyard Navigation with Quadruped Robots

The VINUM project seeks to address the shortage of skilled labor in modern vineyards by introducing a cutting-edge mobile robotic solution. Leveraging the capabilities of the quadruped robot, HyQReal, this system, equipped with arm and vision sensors, offers autonomous navigation and winter pruning of grapevines reducing the need for human intervention. At the heart of this approach lies an architecture that empowers the robot to easily navigate vineyards, identify grapevines with unparalleled accuracy, and approach them for pruning with precision. A state machine drives the process, deftly switching between various stages to ensure seamless and efficient task completion. The system's performance was assessed through experimentation, focusing on waypoint precision and optimizing the robot's workspace for single-plant operations. Results indicate that the architecture is highly reliable, with a mean error of 21.5cm and a standard deviation of 17.6cm for HyQReal. However, improvements in grapevine detection accuracy are necessary for optimal performance. This work is based on a computer-vision-based navigation method for quadruped robots in vineyards, opening up new possibilities for selective task automation. The system's architecture works well in ideal weather conditions, generating and arriving at precise waypoints that maximize the attached robotic arm's workspace. This work is an extension of our short paper presented at the Italian Conference on Robotics and Intelligent Machines (I-RIM).

==> formatting/bibliography-setup.tex <==
\bibliography{ref} 
\bibliographystyle{ieeetr}

==> formatting/do_not_number.tex <==
%include this file in the preamble
%removes numbering from section headings
\setcounter{secnumdepth}{0} % sections are level 1

==> formatting/figures.tex <==
\newcommand{\fig}[3]
    {\begin{figure}
        \centering
        \includegraphics[width=#2in]{#1}
        \caption{#3}
        \label{#3}
     \end{figure}}


\newcommand{\tabl}[2]
    {\begin{table}
        \centering
        {#1}
        \caption{#2}
        \label{#2}
    \end{table}}
    
    
\newcommand{\figref}[1]{(Figure \ref{#1})}

\newcommand{\tableref}[1]{(Table \ref{#1})}

==> formatting/graphics.tex <==
%include this file in the preamble
%Adds images stored in the main file tree
%to use, "\includegraphics{fname.png}[]
\usepackage{graphicx}
\graphicspath{./}

==> formatting/header_footer.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
% \thepage inserts the page number
% [RE, RO] are alignment tabs
% \fancyfoot is also a command 
\fancyhead[RE,RO]{Advertisement Analysis: Surfrider Foundation \thepage}
\renewcommand{\headrulewidth}{0pt}

==> formatting/line_spacing.tex <==
\usepackage{setspace}
%set to 1 for single space, 2 for double space, and so on
\setstretch{1.5}

==> formatting/margins.tex <==
\usepackage[margin=0.5in]{geometry}

==> formatting/table_of_contents_setup.tex <==

%include this file in the preamble
%to use, type in "\tableofcontents" sometime after \begin{document}
\usepackage{color}   %May be necessary if you want to color links
\usepackage{hyperref}
\hypersetup{
    colorlinks=true, %set true if you want colored links
    linktoc=all,     %set to all if you want both sections and subsections linked
    linkcolor=blue,  %choose some color if you want links to stand out
}

==> sections/8_references.tex <==
\printbibliography
